A Principled Self-Referenced Early Stopping Approach for Deep Image Prior

Recently, Deep Image Prior (DIP) has demonstrated strong capabilities for solving inverse imaging problems (IIPs) by optimizing a randomly initialized convolutional neural network in a training-data-free regime. However, DIP suffers from overfitting to noisy measurements due to network over-parameterization, making early stopping (ES) essential. The most successful ES method tracks fluctuations in the running variance of the network output to detect overfitting. However, in many applications, these fluctuations may appear prematurely, leading to unstable reconstructions. In this paper, we first show that nearly optimal DIP early stopping can be achieved when two independent noisy copies of the degraded image are available. Motivated by this observation, and since obtaining two fully independent copies is infeasible, we propose an overfitting detection framework based on constructing pseudo self-referenced images, resulting in three IIP-specific algorithms. Our approach is further supported by theoretical results on single-reference validation, pseudo-validation estimation, and the impact of shared noise. Across different IIPs, ranging from natural image restoration to medical image reconstruction, and under varying noise levels and noise types, our methods consistently outperform existing DIP early stopping approaches, all without requiring an accurate estimate of the noise level.

==> sections/Additional_Experimental_Results.tex <==
\section{Additional Experimental Results}
\label{app:add_exp}

This section provides additional experimental evidence supporting the main results in Section~\ref{sec:experiments}. 
The main paper focuses on four representative quantitative studies and three visualizations. 
Here, we provide complementary results that clarify the behavior of the proposed early-stopping criteria from five aspects: 
(i) analysis of the RGB channel-reference selection used by CSR-ES, 
(ii) additional trajectory and qualitative visualizations, 
(iii) per-image method-specific oracle comparisons on natural and medical images, 
(iv) ablations of MSE-based and bias-based reference scores, and 
(v) sensitivity of ACR-ES to auxiliary noise levels.


\subsection{Analysis of RGB Channel References in CSR-ES}
\label{app:csr_grid}

CSR-ES relies on the observation that different RGB channels of a natural image often share correlated structures. 
The method automatically selects a pseudo-reference channel pair from the noisy observation and uses the corresponding cross-channel consistency curve as a validation signal. 
In this section, we examine all possible RGB channel-reference pairs to verify whether the automatically selected pair is reliable.

Table~\ref{tab:mres_rgb_grid} reports the CSR-ES results over all RGB channel-reference pairs. 
Rows correspond to the pseudo-reference channel $y_j$, while columns correspond to the reconstructed channel $\hat{x}_{t,i}$. 
Each entry shows the stopping iteration selected by the validation curve 
\[
\|\hat{x}_{t,i}-y_j\|^2/n
\]
and the corresponding reconstruction PSNR. 
The highlighted entry denotes the pair automatically selected by CSR-ES using the noisy observation only. 
The oracle result is reported only for evaluation and is not used by CSR-ES.

For Gaussian noise, CSR-ES selects the pair $(\hat{x}_R,y_G)$ and stops at iteration $2373$, achieving $21.2249$ dB, exactly matching the oracle-best PSNR.
For Poisson noise, CSR-ES selects $(\hat{x}_G,y_R)$ and stops at iteration $4980$, again exactly matching the oracle-best PSNR of $22.8460$ dB.
For impulse noise, CSR-ES selects $(\hat{x}_G,y_B)$ and stops at iteration $2348$, achieving $23.5807$ dB, only $0.0427$ dB below the oracle maximum of $23.6234$ dB.
These results demonstrate that the channel similarity reference provides a reliable pseudo-validation signal for early stopping without access to the clean image.

\input{results/table_CSR}



\begin{figure}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/15_Poisson_adam_LR_0.0001_WMV_curve.png}}
\centerline{\scriptsize (a) WMV-ES  curve with ACR-ES training
}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/15_Poisson_adam_LR_0.0001_ACR_curve.png}}
\centerline{\scriptsize (b) ACR-ES  curve with ACR-ES training
}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/L05_Gaussian_adam_LR_0.0001_WMV_curve.png}}
\centerline{\scriptsize (c) WMV-ES  curve with MR-ES training
}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/L05_Gaussian_adam_LR_0.0001_MR_curve.png}}
\centerline{\scriptsize (d) MR-ES  curve with MR-ES training
}
\end{minipage}
\caption{Early stop for image denoising. First row is the nature image from Set18 corrupted by Poisson noise, the second row is the CT image from CT10 corrupted by Gaussian noise.}\label{fig:acr_mr_curve_extra}
\end{figure}

\subsection{Additional Trajectory and Qualitative Results}
\label{app:additional_curves}

The main paper includes representative trajectory plots showing that the proposed criteria select iterations close to the oracle region. 
Here, we provide additional curves and qualitative examples to show that this behavior is consistent across different image types and corruption models.

Figure~\ref{fig:acr_mr_curve_extra} compares WMV-ES with ACR-ES and MR-ES on representative natural and medical images. 
The WMV curve may reach its minimum before the PSNR peak, leading to premature stopping. 
In contrast, the proposed reference-based scores better track the region where the reconstruction quality is close to the oracle.

Figures~\ref{fig:acr_poisson_visual} and~\ref{fig:acr_gaussian_visual} provide qualitative denoising examples under Poisson and Gaussian noise. 
Each figure shows the noisy observation, the auxiliary corrupted references, the reconstruction selected by WMV-ES, the reconstruction selected by ACR-ES, and the oracle reconstruction. 
The selected iteration of ACR-ES is closer to the oracle iteration, and the corresponding reconstruction is visually closer to the oracle-quality result.

\begin{figure}
\centering
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_noisy.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) Poisson noise $y$
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_noisy1.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) Poisson noise $y_1=y+\zeta_1$}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_noisy2.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) Poisson noise $y_2=y+\zeta_2$}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) WMV-ES at Iter. 3069
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) ACR-ES at Iter. 2216}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.8in]{results/img_035_SRF_2_HR_Poisson_max.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) Oracle at Iter. 2307}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/img_035_SRF_2_HR_Poisson_WMV_curve.png}}\vspace{-0.05in}
\centerline{\scriptsize (g) WMV-ES curve with ACR-ES training}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/img_035_SRF_2_HR_Poisson_ACR_curve.png}}\vspace{-0.05in}
\centerline{\scriptsize (h) ACR-ES curve with ACR-ES training}
\end{minipage}
\caption{Image denoising results on Poisson noise. Comparison of WMV-ES and our ACR-ES. }\label{fig:acr_poisson_visual}
\end{figure}
\begin{figure}
\centering
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_noisy.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) Gaussian noise $y$
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_noisy1.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) Gaussian noise $y_1=y+\zeta_1$}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_noisy2.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) Gaussian noise $y_2=y+\zeta_2$}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) WMV-ES at Iter. 534
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) ACR-ES at Iter. 1004}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/face_Gaussian_max.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) Oracle at Iter. 988}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/face_Gaussian_WMV_curve.png}}\vspace{-0.05in}
\centerline{\scriptsize (g) WMV-ES curve with ACR-ES training}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/face_Gaussian_ACR_curve.png}}\vspace{-0.05in}
\centerline{\scriptsize (h) ACR-ES curve with ACR-ES training}
\end{minipage}
\caption{Image denoising results on Gaussian noise. Comparison of WMV-ES and our ACR-ES. }\label{fig:acr_gaussian_visual}
\end{figure}


Figure \ref{fig:ct_acr_gaussian_visual} shows the denoising results of CT image corrupted by the Gaussian noise. We provide the noisy observation, two auxiliary corrupted references, the reconstruction selected by WMV-ES, the reconstruction selected by ACR-ES, and the oracle reconstruction. The corresponding WMV-ES and ACR-ES curves are also given. The selected iteration of ACR-ES is closer to the oracle iteration. Besides, we also present the denoising results of T2 image corrupted by the Impulse noise in Figure \ref{fig:t2_acr_gaussian_visual}. We show the noisy image, the reconstruction selected by WMV-ES, the reconstruction selected by MR-ES, and the oracle reconstruction. The corresponding WMV-ES and MR-ES curves are also given. The selected iteration of MR-ES is closer to the oracle iteration.
\begin{figure}\centering
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_noisy.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) Gaussian noise $y$
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_noisy1.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) Gaussian noise $y_1=y+\zeta_1$}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_noisy2.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) Gaussian noise $y_2=y+\zeta_2$}
\end{minipage}

\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) WMV-ES at Iter. 486
}
\end{minipage} 
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) ACR-ES at Iter. 954}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[width=1.6in]{results/L08_Gaussian_max.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) Oracle at Iter. 812}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/L08_Gaussian_adam_LR_0.0001_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (g) WMV-ES curve with ACR-ES training}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/L08_Gaussian_adam_LR_0.0001_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (h) ACR-ES curve with ACR-ES training}
\end{minipage}
\caption{Image denoising results on Gaussian noise. Comparison of WMV-ES and our ACR-ES. }\label{fig:ct_acr_gaussian_visual}
\end{figure}
\begin{figure}\centering
\begin{minipage}{0.22\linewidth}
\centerline{\includegraphics[width=1.4in]{results/00001983_Impulse_noisy.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) Impulse noise $y$
}
\end{minipage} \hspace{0.15in}
\begin{minipage}{0.22\linewidth}
\centerline{\includegraphics[width=1.4in]{results/00001983_Impulse_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) WMV-ES at Iter. 382
}
\end{minipage} \hspace{0.15in}
\begin{minipage}{0.22\linewidth}
\centerline{\includegraphics[width=1.4in]{results/00001983_Impulse_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) MR-ES at Iter. 1090}
\end{minipage}\hspace{0.18in}
\begin{minipage}{0.22\linewidth}
\centerline{\includegraphics[width=1.4in]{results/00001983_Impulse_max.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) Oracle at Iter. 1243}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/00001983_Impulse_adam_LR_0.0001_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) WMV-ES curve with MR-ES training}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/00001983_Impulse_adam_LR_0.0001_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) MR-ES curve with MR-ES training}
\end{minipage}
\caption{Image denoising results on Impulse noise. Comparison of WMV-ES and our MR-ES. }\label{fig:t2_acr_gaussian_visual}
\end{figure}

Moreover, we also present the comparison of different training methods among the original DIP, the proposed ACR-ES, and the MR-ES training in Figure \ref{fig:3train}. We test a single image from the CT10 dataset under three different noise types: Gaussian, Poisson, and Impulse. 
From the results, we know that our ACR-ES and MR-ES do not change the original DIP training.  


\begin{figure}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Gaussian_adam_LR_0.0001_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) WMV-ES curve with original DIP training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Gaussian_adam_LR_0.0001_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) ACR-ES curve with ACR-ES training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Gaussian_adam_LR_0.0001_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) MR-ES curve with MR-ES training
}
\end{minipage}

\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Poisson_adam_LR_0.0001_WMV_dip.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) WMV-ES curve with original DIP training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Poisson_adam_LR_0.0001_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) ACR-ES curve with ACR-ES training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Poisson_adam_LR_0.0001_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) MR-ES curve with MR-ES training
}
\end{minipage}

\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Impulse_adam_LR_0.0001_WMV.png}}\vspace{-0.05in}
\centerline{\scriptsize (g) WMV-ES curve with original DIP training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Impulse_adam_LR_0.0001_ACR.png}}\vspace{-0.05in}
\centerline{\scriptsize (h) ACR-ES curve with ACR-ES training
}
\end{minipage}\hspace{0.1in}
\begin{minipage}{0.31\linewidth}
\centerline{\includegraphics[width=1.85in]{results/L01_Impulse_adam_LR_0.0001_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (i) MR-ES curve with MR-ES training
}
\end{minipage}
\caption{Comparison of different training curves of WMV-ES and the proposed reference-based stopping criteria. Test on CT01 image corrupted by Gaussian noise in the first row; Poisson noise in the second row; and Impulse noise in the third row.}\label{fig:3train}
\end{figure}







We further compare the proposed reference-based stopping criteria with SURE-ES and WMV-ES through representative stopping-score trajectories.
Although SURE provides an unbiased estimate of the reconstruction risk under specific Gaussian-noise assumptions, its empirical minimum does not always coincide with the oracle stopping region of DIP optimization.
Figure~\ref{fig:sure_curve_extra} shows examples on a natural image and a medical image corrupted by Gaussian noise.
For the natural image, we compare the SURE curve on the original DIP trajectory with WMV-ES and MR-ES curves on the corresponding reference-based training trajectories.
For the medical image, we compare SURE-ES with the stopping curve obtained under ACR-ES training.
These examples show that the proposed reference-based stopping signals are better aligned with the near-oracle region than SURE-ES or WMV-ES in these representative cases.
This complements the quantitative comparisons in the main paper and further illustrates the robustness of the proposed stopping principle across image domains and training trajectories.

\begin{figure}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/SURE_gaussian_starfish.png}}\vspace{-0.05in}
\centerline{\scriptsize (a) SURE curve with original DIP training
}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/ACR_gaussian_starfish.png}}\vspace{-0.05in}
\centerline{\scriptsize (b) WMV-ES curve with ACR-ES training
}
\end{minipage}

\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/Starfish_gaussian_MR.png}}\vspace{-0.05in}
\centerline{\scriptsize (c) WMV-ES curve with MR-ES training
}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/Starfish_gaussian_MR_curve.png}}\vspace{-0.05in}
\centerline{\scriptsize (d) MR-ES curve with MR-ES training
}
\end{minipage}


\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/SURE_T2_gaussian.png}}\vspace{-0.05in}
\centerline{\scriptsize (e) SURE curve with original DIP training
}
\end{minipage}\hspace{0.35in}
\begin{minipage}{0.45\linewidth}
\centerline{\includegraphics[width=2.8in]{results/ACR_T2_gaussian.png}}\vspace{-0.05in}
\centerline{\scriptsize (f) WMS-ES curve with ACR training
}
\end{minipage}
\caption{Comparison of different training curves of SURE, WMV-ES, and the proposed reference-based stopping criteria. First and second row are the nature image from Set3 corrupted by Gaussian noise, the third row is the CT image from T2-20 corrupted by Gaussian noise.}\label{fig:sure_curve_extra}
\end{figure}



\begin{table}[t]
\centering
\caption{
Representative early-stopping comparison on selected natural images. 
Each PSNR entry is reported as ES PSNR (Oracle PSNR), where the oracle PSNR is computed from the corresponding training trajectory of each method. 
Gap denotes Oracle PSNR minus ES PSNR; a smaller Gap indicates a more accurate stopping point.
}
\label{tab:representative_es_gap}
\small
\setlength{\tabcolsep}{4.2pt}
\renewcommand{\arraystretch}{1.18}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc cc cc cc cc}
\toprule
\multirow{3}{*}{Noise}
& \multirow{3}{*}{Image}
& \multicolumn{2}{c}{SURE-ES}
& \multicolumn{2}{c}{WMV-ES}
& \multicolumn{2}{c}{MR-ES}
& \multicolumn{2}{c}{CSR-ES}
& \multicolumn{2}{c}{ACR-ES} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
\cmidrule(lr){11-12}
&
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$ \\
\midrule

\multirow{10}{*}{Gaussian}
& Leaves
& 20.06 (21.43) & 1.37
& 20.64 (20.89) & 0.25
& 20.62 (20.84) & 0.22
& 20.59 (20.70) & 0.11
& \textbf{20.62 (20.70)} & \textbf{0.08} \\
& Starfish
& 21.31 (22.04) & 0.73
& 18.96 (21.73) & 2.77
& 21.23 (21.72) & 0.49
& 21.39 (21.69) & 0.30
& \textbf{21.52 (21.69)} & \textbf{0.17} \\
& Baboon
& 19.50 (19.92) & 0.42
& 18.30 (19.63) & 1.33
& 19.37 (19.62) & 0.25
& 19.22 (19.50) & 0.28
& \textbf{19.42 (19.50)} & \textbf{0.08} \\
& Barbara
& 21.81 (23.01) & 1.20
& 21.61 (22.66) & 1.05
& 22.30 (22.58) & 0.29
& \textbf{22.46 (22.55)} & \textbf{0.09}
& 22.21 (22.55) & 0.34 \\
& Coastguard
& 22.82 (23.30) & 0.48
& 21.87 (23.10) & 1.22
& 21.95 (22.75) & 0.80
& \textbf{22.77 (22.86)} & \textbf{0.09}
& 22.59 (22.86) & 0.27 \\
& Comic
& 18.46 (20.58) & 2.11
& 17.94 (20.07) & 2.12
& 19.76 (19.86) & 0.11
& 19.81 (19.94) & 0.13
& \textbf{19.91 (19.94)} & \textbf{0.03} \\
& Face
& 22.03 (22.72) & 0.69
& 22.39 (22.66) & 0.27
& 22.26 (22.49) & 0.23
& 22.27 (22.51) & 0.24
& \textbf{22.42 (22.51)} & \textbf{0.09} \\
& Flowers
& 21.93 (22.35) & 0.42
& 21.07 (21.90) & 0.83
& 21.39 (21.72) & 0.34
& \textbf{21.62 (21.82)} & \textbf{0.21}
& 21.61 (21.82) & 0.21 \\
& Foreman
& 20.36 (24.06) & 3.71
& 23.50 (23.88) & 0.38
& 23.47 (23.79) & 0.31
& \textbf{23.71 (23.82)} & \textbf{0.12}
& 23.63 (23.82) & 0.19 \\
& Zebra
& 22.59 (23.04) & 0.45
& 22.09 (22.61) & 0.52
& 22.28 (22.49) & 0.22
& \textbf{22.33 (22.45)} & \textbf{0.12}
& 22.13 (22.45) & 0.32 \\
\midrule

\multirow{10}{*}{Poisson}
& Leaves
& 20.39 (20.83) & 0.44 
& 20.33 (20.47) & 0.14
& 20.32 (20.43) & 0.11
& \textbf{20.92 (21.03)} & \textbf{0.11}
& 20.89 (21.03) & 0.13 \\
& Starfish
& 22.92 (23.16) & 0.24 
& 22.15 (22.69) & 0.54
& 22.69 (22.86) & 0.18
& 23.40 (23.51) & 0.11
& \textbf{23.42 (23.51)} & \textbf{0.09} \\
& Baboon
& 18.90 (20.97) & 2.07
& 18.66 (20.56) & 1.90
& 20.37 (20.54) & 0.17
& \textbf{20.46 (20.54)} & \textbf{0.08}
& 20.41 (20.54) & 0.13 \\
& Barbara
& 23.92 (24.02) & 0.10
& 23.29 (23.56) & 0.27
& 23.21 (23.48) & 0.27
& 24.75 (24.85) & 0.11
& 24.78 (24.85) & 0.07 \\
& Coastguard
& 24.04 (24.47) & 0.43
& 22.93 (23.83) & 0.91
& 23.58 (23.75) & 0.17
& \textbf{24.62 (24.75)} & \textbf{0.13}
& 24.61 (24.75) & 0.14 \\
& Comic
& 19.04 (20.90) & 1.87
& 17.75 (20.35) & 2.59
& 19.84 (20.39) & 0.55
& 21.38 (21.52) & 0.14
& \textbf{21.40 (21.52)} & \textbf{0.12} \\
& Face
& 26.30 (26.49) & 0.19
& 25.50 (26.17) & 0.67
& 25.89 (26.27) & 0.38
& 26.59 (26.79) & 0.20
& \textbf{26.73 (26.79)} & \textbf{0.06} \\
& Flowers
& 21.71 (23.91) & 2.20
& 22.89 (23.55) & 0.65
& 22.99 (23.33) & 0.34
& \textbf{24.47 (24.54)} & \textbf{0.07}
& 24.39 (24.54) & 0.14 \\
& Foreman
& 23.27 (23.62) & 0.34
& 23.15 (23.31) & 0.15
& 23.07 (23.25) & 0.18
& 23.69 (23.84) & 0.15
& \textbf{23.70 (23.84)} & \textbf{0.14} \\
& Zebra
& 22.53 (24.68) & 2.14
& 23.95 (24.11) & 0.17
& \textbf{24.25 (24.31)} & \textbf{0.06}
& 24.90 (25.24) & 0.33
& 25.01 (25.24) & 0.22 \\
\midrule

\multirow{10}{*}{Impulse}
& Leaves
& 17.79 (23.19) & 5.40
& 22.18 (22.34) & 0.16
& 21.59 (22.25) & 0.66
& \textbf{22.12 (22.17)} & \textbf{0.04}
& 21.88 (22.17) & 0.28 \\
& Starfish
& 19.10 (23.92) & 4.82
& 22.68 (23.32) & 0.64
& 22.99 (23.11) & 0.13
& 23.04 (23.38) & 0.34
& \textbf{23.12 (23.38)} & \textbf{0.26} \\
& Baboon
& 20.74 (21.00) & 0.27
& 18.53 (20.50) & 1.97
& 20.03 (20.31) & 0.28
& \textbf{20.34 (20.36)} & \textbf{0.02}
& 20.30 (20.36) & 0.06 \\
& Barbara
& 23.69 (24.17) & 0.49
& 23.32 (23.90) & 0.58
& 23.34 (23.69) & 0.31
& \textbf{23.49 (23.65)} & \textbf{0.16}
& 23.32 (23.65) & 0.33 \\
& Coastguard
& 20.56 (24.65) & 4.09
& 23.05 (24.26) & 1.22
& 23.95 (24.18) & 0.23
& \textbf{24.12 (24.28)} & \textbf{0.15}
& 23.68 (24.28) & 0.60 \\
& Comic
& 19.86 (22.15) & 2.30
& 18.14 (21.45) & 3.31
& 21.00 (21.17) & 0.17
& \textbf{20.98 (21.13)} & \textbf{0.16}
& 20.93 (21.13) & 0.20 \\
& Face
& 16.85 (24.86) & 8.01
& 24.27 (24.81) & 0.54
& 24.18 (24.75) & 0.57
& \textbf{24.59 (24.75)} & \textbf{0.17}
& 23.73 (24.75) & 1.02 \\
& Flowers
& 21.87 (23.78) & 1.91
& 22.63 (23.23) & 0.60
& 22.90 (23.10) & 0.20
& \textbf{22.98 (23.11)} & \textbf{0.13}
& 22.75 (23.11) & 0.36 \\
& Foreman
& 20.17 (26.36) & 6.19
& 25.68 (26.03) & 0.35
& 25.52 (25.90) & 0.38
& \textbf{25.96 (26.07)} & \textbf{0.11}
& 25.41 (26.07) & 0.66 \\
& Zebra
& 22.86 (24.99) & 2.13
& 23.98 (24.34) & 0.36
& 23.90 (24.14) & 0.24
& \textbf{24.00 (24.24)} & \textbf{0.24}
& 23.79 (24.24) & 0.44 \\
\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{
Representative early-stopping comparison on selected medical images. 
Each PSNR entry is reported as ES PSNR (Oracle PSNR), where the oracle PSNR is computed from the corresponding training trajectory of each method. 
Gap denotes Oracle PSNR minus ES PSNR; a smaller Gap indicates a more accurate stopping point.
}
\label{tab:representative_medical_es_gap}
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.18}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcc cc cc cc}
\toprule
\multirow{3}{*}{Noise}
& \multirow{3}{*}{Image}
& \multicolumn{2}{c}{SURE-ES}
& \multicolumn{2}{c}{WMV-ES}
& \multicolumn{2}{c}{MR-ES}
& \multicolumn{2}{c}{ACR-ES} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
\cmidrule(lr){7-8}
\cmidrule(lr){9-10}
&
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$
& \makecell{PSNR\\(Oracle)} & Gap $\downarrow$ \\
\midrule

\multirow{10}{*}{Gaussian}
& CT01
& 19.34 (20.92) & 1.59
& 19.46 (20.49) & 1.03
& \textbf{20.35 (20.47)} & \textbf{0.12}
& 20.52 (20.68) & 0.16 \\
% & CT04
% & 15.38 (21.61) & 6.24
% & 21.11 (21.59) & 0.48
% & 21.06 (21.33) & 0.27
% & \textbf{21.29 (21.44)} & \textbf{0.15} \\
& CT05
& 20.42 (20.79) & 0.37
& 19.93 (20.95) & 1.02
& 20.47 (20.67) & 0.20
& \textbf{20.49 (20.63)} & \textbf{0.14} \\
& CT06
& 18.04 (20.50) & 2.46
& 19.95 (20.64) & 0.69
& 19.78 (20.25) & 0.47
& \textbf{20.22 (20.45)} & \textbf{0.23} \\
& CT08
& 15.26 (21.64) & 6.38
& 21.12 (21.41) & 0.28
& 20.12 (21.17) & 1.05
& \textbf{21.11 (21.30)} & \textbf{0.20} \\
& CT09
& 16.39 (20.55) & 4.17
& 20.16 (20.57) & 0.40
& 19.85 (20.21) & 0.36
& \textbf{19.96 (20.20)} & \textbf{0.24} \\
& T2-23
& 19.58 (19.76) & 0.19
& 16.77 (19.57) & 2.80
& 19.23 (19.64) & 0.41
& \textbf{19.37 (19.50)} & \textbf{0.13} \\
& T2-633
& 15.31 (19.93) & 4.62
& 15.87 (19.94) & 4.07
& \textbf{19.72 (19.76)} & \textbf{0.04}
& 19.58 (19.75) & 0.17 \\
& T2-1173
& 15.27 (19.88) & 4.61
& 17.17 (19.87) & 2.70
& 19.68 (19.85) & 0.17
& \textbf{19.63 (19.79)} & \textbf{0.17} \\
& T2-1783
& 15.60 (19.86) & 4.26
& 16.72 (19.72) & 3.00
& 19.23 (19.53) & 0.30
& \textbf{19.40 (19.58)} & \textbf{0.18} \\
& T2-2273
& 18.52 (20.06) & 1.54
& 16.72 (19.95) & 3.23
& 19.71 (19.79) & 0.08
& \textbf{19.86 (19.94)} & \textbf{0.08} \\
\midrule

\multirow{10}{*}{Poisson}
& CT01
& 19.79 (25.66) & 5.87
& 23.84 (26.02) & 2.18
& 24.05 (25.05) & 1.01
& \textbf{26.07 (26.46)} & \textbf{0.40} \\
% & CT04
% & 20.41 (27.33) & 6.91
% & 24.91 (26.71) & 1.80
% & 24.74 (26.87) & 2.12
% & \textbf{27.36 (27.98)} & \textbf{0.62} \\
& CT05
& 22.71 (27.15) & 4.44
& 24.17 (28.03) & 3.86
& 24.63 (27.12) & 2.48
& \textbf{29.26 (29.60)} & \textbf{0.35} \\
& CT06
& 20.88 (26.51) & 5.63
& 22.36 (26.11) & 3.75
& \textbf{25.30 (26.00)} & \textbf{0.70}
& 25.94 (27.18) & 1.24 \\
& CT08
& 22.26 (26.25) & 3.99
& 24.27 (25.94) & 1.67
& 23.99 (25.58) & 1.59
& \textbf{26.28 (26.39)} & \textbf{0.10} \\
& CT09
& 18.82 (26.31) & 7.49
& 22.76 (26.34) & 3.57
& 23.86 (26.11) & 2.25
& \textbf{26.86 (27.63)} & \textbf{0.77} \\
& T2-23
& 24.44 (25.97) & 1.53
& 18.55 (25.96) & 7.41
& 23.35 (25.87) & 2.52
& \textbf{25.60 (26.92)} & \textbf{1.32} \\
& T2-633
& 17.41 (25.60) & 8.18
& 17.95 (26.55) & 8.60
& 23.14 (26.48) & 3.34
& \textbf{27.11 (28.14)} & \textbf{1.04} \\
& T2-1173
& 24.59 (25.99) & 1.39
& 20.30 (27.37) & 7.07
& 23.48 (26.66) & 3.17
& \textbf{27.29 (28.25)} & \textbf{0.96} \\
& T2-1783
& 23.37 (24.80) & 1.43
& 17.91 (25.62) & 7.71
& 23.00 (25.45) & 2.45
& \textbf{25.12 (26.36)} & \textbf{1.24} \\
& T2-2273
& 22.56 (25.98) & 3.42
& 17.94 (25.91) & 7.97
& 22.86 (25.74) & 2.88
& \textbf{25.94 (26.95)} & \textbf{1.01} \\
\midrule

\multirow{10}{*}{Impulse}
& CT01
& 14.95 (22.98) & 8.03
& 21.23 (22.90) & 1.66
& 22.38 (22.74) & 0.36
& \textbf{22.14 (22.38)} & \textbf{0.24} \\
% & CT04
% & 15.25 (24.64) & 9.39
% & 23.18 (24.64) & 1.46
% & \textbf{23.98 (24.38)} & \textbf{0.40}
% & 23.86 (24.38) & 0.52 \\
& CT05
& 14.50 (22.92) & 8.42
& 23.04 (23.95) & 0.92
& \textbf{22.81 (23.06)} & \textbf{0.26}
& 22.45 (23.04) & 0.59 \\
& CT06
& 14.39 (23.26) & 8.87
& 21.15 (23.05) & 1.90
& 22.09 (22.83) & 0.74
& \textbf{22.02 (22.35)} & \textbf{0.32} \\
& CT08
& 15.71 (24.26) & 8.55
& 23.32 (23.85) & 0.53
& 23.84 (24.10) & 0.25
& \textbf{23.43 (23.67)} & \textbf{0.24} \\
& CT09
& 14.63 (23.24) & 8.62
& 21.00 (22.85) & 1.86
& 22.56 (22.86) & 0.30
& \textbf{22.49 (22.75)} & \textbf{0.26} \\
& T2-23
& 14.64 (21.99) & 7.35
& 18.15 (22.01) & 3.86
& 21.40 (21.88) & 0.48
& \textbf{21.55 (21.67)} & \textbf{0.12} \\
& T2-633
& 14.51 (22.73) & 8.22
& 21.90 (22.53) & 0.63
& \textbf{22.19 (22.31)} & \textbf{0.12}
& 22.14 (22.26) & 0.13 \\
& T2-3
& 14.18 (22.60) & 8.42
& 19.81 (22.97) & 3.16
& \textbf{22.10 (22.34)} & \textbf{0.24}
& 21.30 (21.96) & 0.67 \\
& T2-1783
& 14.15 (21.98) & 7.83
& 18.02 (22.02) & 4.00
& 21.51 (21.80) & 0.29
& \textbf{21.21 (21.45)} & \textbf{0.24} \\
& T2-2273
& 14.20 (22.30) & 8.10
& 19.18 (22.21) & 3.03
& \textbf{21.86 (22.07)} & \textbf{0.21}
& 20.48 (21.92) & 1.43 \\
\bottomrule
\end{tabular}}
\end{table}

\subsection{Full Method-specific Oracle Comparisons}
\label{app:oracle_full}

Section~\ref{subsec:oracle_analysis} summarizes the method-specific oracle analysis using group-level averages.
Here, we provide the full per-image comparisons on representative natural and medical images.
The purpose of this analysis is to verify that the proposed criteria reduce the PSNR Gap by selecting stopping points closer to the oracle region, rather than by lowering the attainable oracle PSNR of the corresponding trajectory.

Tables~\ref{tab:representative_es_gap} and~\ref{tab:representative_medical_es_gap} report per-image results on natural and medical images, respectively.
Each entry is written as ES PSNR (Oracle PSNR), where the oracle PSNR is computed from the corresponding training trajectory of each method.
Thus, the selected reconstruction quality and the best attainable quality along the same method-specific trajectory can be compared simultaneously.

Table~\ref{tab:representative_es_gap} reports results on selected natural images under Gaussian, Poisson, and impulse noise.
Across different images and noise types, CSR-ES and ACR-ES generally achieve smaller oracle gaps than SURE-ES and WMV-ES while maintaining comparable oracle PSNR values.
This indicates that the improvement is not caused by degrading the reconstruction trajectory.
Instead, the proposed color-image criteria provide stopping signals that more accurately identify the near-oracle region of the corresponding trajectory.

Table~\ref{tab:representative_medical_es_gap} reports the corresponding results on selected CT and T2 images.
Since CSR-ES relies on RGB channel consistency, it is not applicable to these grayscale medical images.
MR-ES and ACR-ES instead provide reference-based stopping signals through mask-based and auxiliary-corruption-based references.
For Gaussian and impulse noise, MR-ES and ACR-ES generally select iterations close to their own oracle trajectories.
For Poisson noise, where the corruption is signal-dependent and the mask-reference signal can be less stable, ACR-ES often achieves substantially smaller gaps than SURE-ES, WMV-ES, and MR-ES.
These per-image results are consistent with the averaged trends in the main paper and further support the conclusion that the proposed criteria improve stopping accuracy by better identifying the best attainable region along each trajectory.

\subsection{Ablation Study: MSE-based and Bias-based Reference Scores}
\label{app:score_ablation}

We next study the effect of different reference scores. 
The proposed framework uses different reference constructions for natural color images and grayscale medical images. 
For natural color images, ACR-ES uses a bias-based cross-reference score. 
For grayscale medical images, MR-ES uses an MSE-based mask-reference score. 
This section justifies these choices.

For natural color images, we compare bias-based and MSE-based variants of ACR-ES. 
Table~\ref{tab:acr_bias_vs_mse_natural} shows that the bias-based ACR-ES consistently reduces the PSNR Gap compared with the MSE-based variant, especially under Gaussian and impulse noise. 
This suggests that, for RGB images, cross-reference bias information captures useful stopping behavior beyond direct MSE consistency.




\begin{table}[t]
\centering
\caption{Comparison between bias-based and MSE-based ACR-ES on natural image datasets. 
PSNR and PSNR Gap are reported as mean $\pm$ standard deviation across images. 
Positive $\Delta$ Gap indicates that ACR-ES (Bias) is closer to the oracle stopping point.}
\label{tab:acr_bias_vs_mse_natural}
\small
\setlength{\tabcolsep}{5.2pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Noise}
& \multirow{2}{*}{Dataset}
& \multicolumn{2}{c}{ACR-ES (Bias)}
& \multicolumn{2}{c}{ACR-ES (MSE)}
& \multirow{2}{*}{$\Delta$ Gap $\uparrow$} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&
& PSNR $\uparrow$ & Gap $\downarrow$
& PSNR $\uparrow$ & Gap $\downarrow$
& \\
\midrule

\multirow{4}{*}{Gaussian}
& Set14
& \textbf{22.26($\pm$1.71)} & \textbf{0.25($\pm$0.13)}
& 21.44($\pm$1.67) & 1.06($\pm$0.79)
& \cellcolor{green!8}0.81 \\
& Set18
& \textbf{22.33($\pm$1.52)} & \textbf{0.21($\pm$0.12)}
& 21.65($\pm$0.84) & 0.89($\pm$1.24)
& \cellcolor{green!8}0.68 \\
& CBSD68
& \textbf{22.33($\pm$1.99)} & \textbf{0.30($\pm$0.28)}
& 21.15($\pm$1.58) & 1.48($\pm$1.44)
& \cellcolor{green!8}1.18 \\
& Urban100
& \textbf{21.36($\pm$1.31)} & \textbf{0.20($\pm$0.10)}
& 20.60($\pm$1.01) & 0.97($\pm$0.65)
& \cellcolor{green!8}0.76 \\
\addlinespace[2pt]
\midrule

\multirow{4}{*}{Poisson}
& Set14
& \textbf{24.52($\pm$2.35)} & \textbf{0.11($\pm$0.05)}
& 24.52($\pm$2.35) & 0.11($\pm$0.07)
& \cellcolor{green!8}0.00 \\
& Set18
& \textbf{26.55($\pm$2.33)} & \textbf{0.15($\pm$0.10)}
& 26.53($\pm$2.32) & 0.17($\pm$0.11)
& \cellcolor{green!8}0.02 \\
& CBSD68
& \textbf{24.66($\pm$2.33)} & \textbf{0.14($\pm$0.09)}
& 24.66($\pm$2.32) & 0.14($\pm$0.08)
& \cellcolor{green!8}0.00 \\
& Urban100
& 24.08($\pm$1.66) & 0.18($\pm$0.12)
& \textbf{24.09($\pm$1.64)} & \textbf{0.17($\pm$0.10)}
& \cellcolor{red!6}-0.01 \\
\addlinespace[2pt]
\midrule

\multirow{4}{*}{Impulse}
& Set14
& \textbf{23.65($\pm$1.74)} & \textbf{0.49($\pm$0.23)}
& 22.50($\pm$1.77) & 1.64($\pm$1.56)
& \cellcolor{green!8}1.15 \\
& Set18
& \textbf{24.09($\pm$1.52)} & \textbf{0.53($\pm$0.21)}
& 23.11($\pm$0.97) & 1.50($\pm$0.76)
& \cellcolor{green!8}0.97 \\
& CBSD68
& \textbf{23.63($\pm$2.02)} & \textbf{0.44($\pm$0.25)}
& 22.29($\pm$1.36) & 1.78($\pm$1.08)
& \cellcolor{green!8}1.34 \\
& Urban100
& \textbf{22.86($\pm$1.42)} & \textbf{0.34($\pm$0.17)}
& 22.23($\pm$1.08) & 0.97($\pm$0.66)
& \cellcolor{green!8}0.63 \\

\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{Comparison between the MSE-based and bias-based mask-reference early stopping criteria on medical datasets. 
PSNR and PSNR Gap are reported as mean $\pm$ standard deviation across images. 
Positive $\Delta$ Gap=Gap(Bias)-Gap(MSE) indicates that the MSE-based criterion is closer to the oracle stopping point.}
\label{tab:mse_vs_bias_medical}
\small
\setlength{\tabcolsep}{5.5pt}
\renewcommand{\arraystretch}{1.15}
% \resizebox{\linewidth}{!}
{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Noise}
& \multirow{2}{*}{Dataset}
& \multicolumn{2}{c}{MR-ES (MSE)}
& \multicolumn{2}{c}{MR-ES (Bias)}
& \multirow{2}{*}{$\Delta$ Gap $\uparrow$} \\
\cmidrule(lr){3-4}
\cmidrule(lr){5-6}
&
& PSNR $\uparrow$ & Gap $\downarrow$
& PSNR $\uparrow$ & Gap $\downarrow$
& \\
\midrule

\multirow{4}{*}{Gaussian}
& MRI15
& \textbf{21.60($\pm$0.69)} & \textbf{0.41($\pm$0.29)}
& 19.69($\pm$1.69) & 2.33($\pm$1.74)
& \cellcolor{green!8}1.92 \\
& CT10
& \textbf{20.22($\pm$0.47)} & \textbf{0.35($\pm$0.28)}
& 19.66($\pm$1.36) & 0.92($\pm$1.26)
& \cellcolor{green!8}0.57 \\
& PD20
& \textbf{19.94($\pm$0.36)} & \textbf{0.33($\pm$0.24)}
& 18.03($\pm$0.92) & 2.24($\pm$0.93)
& \cellcolor{green!8}1.91 \\
& T2-20
& \textbf{19.62($\pm$0.19)} & \textbf{0.16($\pm$0.09)}
& 18.33($\pm$1.01) & 1.45($\pm$0.98)
& \cellcolor{green!8}1.29 \\
\addlinespace[2pt]
\midrule

\multirow{4}{*}{Poisson}
& MRI15
& \textbf{24.78($\pm$1.27)} & \textbf{1.35($\pm$1.04)}
& 23.33($\pm$1.83) & 2.80($\pm$1.65)
& \cellcolor{green!8}1.45 \\
& CT10
& \textbf{24.56($\pm$1.30)} & \textbf{2.03($\pm$0.85)}
& 23.36($\pm$1.71) & 3.24($\pm$1.60)
& \cellcolor{green!8}1.21 \\
& PD20
& \textbf{21.15($\pm$0.37)} & 4.49($\pm$0.37)
& 21.29($\pm$0.47) & \textbf{4.34($\pm$0.36)}
& \cellcolor{red!6}-0.15 \\
& T2-20
& 23.26($\pm$0.47) & 3.05($\pm$0.36)
& \textbf{23.53($\pm$0.78)} & \textbf{2.78($\pm$0.72)}
& \cellcolor{red!6}-0.27 \\
\addlinespace[2pt]
\midrule

\multirow{4}{*}{Impulse}
& MRI15
& \textbf{23.49($\pm$0.52)} & \textbf{0.46($\pm$0.47)}
& 18.98($\pm$2.91) & 4.96($\pm$2.96)
& \cellcolor{green!8}4.50 \\
& CT10
& \textbf{22.82($\pm$0.70)} & \textbf{0.31($\pm$0.17)}
& 16.77($\pm$1.81) & 6.36($\pm$1.50)
& \cellcolor{green!8}6.05 \\
& PD20
& \textbf{23.12($\pm$0.28)} & \textbf{0.26($\pm$0.19)}
& 16.51($\pm$1.28) & 6.87($\pm$1.34)
& \cellcolor{green!8}6.61 \\
& T2-20
& \textbf{21.89($\pm$0.26)} & \textbf{0.31($\pm$0.16)}
& 16.72($\pm$1.95) & 5.48($\pm$1.93)
& \cellcolor{green!8}5.17 \\
\bottomrule
\end{tabular}}
\end{table}


For grayscale medical images, we compare MSE-based and bias-based variants of MR-ES. 
Table~\ref{tab:mse_vs_bias_medical} shows that the MSE-based mask-reference criterion is generally more reliable than the bias-based variant. 
This is expected because single-channel medical images do not provide the same multi-channel structure as RGB images, making direct mask-reference consistency a more stable validation signal.

Together, these ablations justify the design used in the main paper: bias-based ACR-ES for natural color images and MSE-based MR-ES for grayscale medical images.




\begin{table}[t]
\centering
\caption{Sensitivity of ACR-ES on Set3 to the additional noise level $c$. 
Results are reported as mean $\pm$ standard deviation across images. 
PSNR Gap denotes the difference between Oracle PSNR and ACR-ES PSNR.
For Gaussian noise, the level of noise in the observation $y$ is $\sigma=0.26$ and the level of noise added to the augmented channels is $\tau=1.25\sigma+0.1c$.
For Poisson noise, the noise  in $y$ follows $\mathcal{P}(\lambda)$  with $\lambda=10$ and the noise  added to augmented channel follows $\mathcal{P}(\tau)$ with $\tau=1.25\lambda+c$.
For impulse noise, the probability of measurement corruption is $p=0.1$ in the observation $y$ and $\tau=1.25p+0.1c$ in the augmented channel.
}
\label{tab:set3c_acr_s_ablation}
\small
\setlength{\tabcolsep}{7pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{llccc}
\toprule
Noise 
& $c$ 
& \makecell{ACR-ES\\PSNR $\uparrow$}
& \cellcolor{gray!10}\makecell{Oracle\\PSNR $\uparrow$}
& \makecell{Gap $\downarrow$} \\
\midrule

\multirow{4}{*}{Gaussian}
& $0$    & 21.44($\pm$0.78) & \cellcolor{gray!10}21.55($\pm$0.80) & \textbf{0.11($\pm$0.05)} \\
& $0.10$ & 21.42($\pm$0.84) & \cellcolor{gray!10}21.56($\pm$0.77) & 0.14($\pm$0.08) \\
& $0.15$ & 21.34($\pm$0.85) & \cellcolor{gray!10}21.54($\pm$0.80) & 0.20($\pm$0.06) \\
& $0.20$ & \textbf{21.44($\pm$0.87)} & \cellcolor{gray!10}21.55($\pm$0.86) & \textbf{0.11($\pm$0.08)} \\
\midrule

\multirow{4}{*}{Poisson}
& $0$    & 22.91($\pm$1.82) & \cellcolor{gray!10}23.05($\pm$1.84) & 0.14($\pm$0.06) \\
& $0.10$ & \textbf{23.00($\pm$1.80)} & \cellcolor{gray!10}23.06($\pm$1.74) & \textbf{0.06($\pm$0.06)} \\
& $0.15$ & 22.81($\pm$1.73) & \cellcolor{gray!10}22.97($\pm$1.74) & 0.17($\pm$0.09) \\
& $0.20$ & 22.89($\pm$1.66) & \cellcolor{gray!10}23.07($\pm$1.69) & 0.18($\pm$0.18) \\
\midrule

\multirow{4}{*}{Impulse}
& $0$    & 22.72($\pm$0.73) & \cellcolor{gray!10}23.05($\pm$0.77) & 0.33($\pm$0.10) \\
& $0.10$ & \textbf{22.84($\pm$0.62)} & \cellcolor{gray!10}22.99($\pm$0.63) & \textbf{0.14($\pm$0.08)} \\
& $0.15$ & 22.81($\pm$0.65) & \cellcolor{gray!10}22.97($\pm$0.60) & 0.16($\pm$0.06) \\
& $0.20$ & 22.73($\pm$0.62) & \cellcolor{gray!10}22.95($\pm$0.63) & 0.22($\pm$0.01) \\

\bottomrule
\end{tabular}
\end{table}
\begin{table}[t]
\centering
\caption{
Sensitivity of ACR-ES on Set3 to auxiliary-noise mismatch under Gaussian noise.
Each entry is reported as ES PSNR (Oracle PSNR). 
The default setting used throughout the paper is $\tau_1=\tau_2=1.25\sigma$, highlighted in purple.
Off-diagonal entries correspond to mismatched auxiliary noise levels $\tau_1\neq \tau_2$. 
{
ACR-ES uses the bias score $\mathrm{bias}(y_2,\hat{x}_1)$.
Gray cells denote matched but non-default settings $\tau_1=\tau_2$.
}
}
\label{tab:n1_n2_mismatch_acr_psnr}
\small
\setlength{\tabcolsep}{8pt}
\renewcommand{\arraystretch}{1.20}
\resizebox{0.72\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\diagbox[width=5.8em,height=2.4em]{$\tau_2$}{$\tau_1$}
& $1.0\sigma$
& $1.25\sigma$
& $1.5\sigma$ \\
\midrule

$1.0\sigma$
& \cellcolor{gray!10}20.73 (21.83)
& 21.46 (21.60)
& \textbf{21.65 (21.65)} \\

$1.25\sigma$
& 21.19 (21.69)
& \cellcolor{blue!8}\textbf{21.52 (21.69)}
& \textbf{21.52 (21.69)} \\

$1.5\sigma$
& 20.73 (21.68)
& \textbf{21.34 (21.68)}
& \cellcolor{gray!10}21.32 (21.65) \\

\bottomrule
\end{tabular}}

\end{table}


\subsection{Sensitivity to Auxiliary Noise Levels}
\label{app:aux_sensitivity}

ACR-ES constructs auxiliary corrupted observations and therefore introduces auxiliary noise levels. 
A natural question is whether the method requires precise tuning of these levels. 
In the main experiments, we use the default noise level setting
\[
\tau_1=\tau_2=1.25\sigma,
\]
where $\sigma$ denotes the original noise level. 
Here, we study the sensitivity of ACR-ES to both auxiliary-noise magnitude and mismatch.

Table~\ref{tab:set3c_acr_s_ablation} studies the effect of varying the auxiliary noise magnitude by setting $\tau_1=\tau_2=1.25\sigma+c$ under Gaussian, Poisson, and impulse noise. 
The PSNR and PSNR Gap remain stable across different values of $c$, showing that ACR-ES is not overly sensitive to the precise auxiliary-noise strength.


We further evaluate mismatched auxiliary noise levels in Table~\ref{tab:n1_n2_mismatch_acr_psnr}, where $\tau_1$ and $\tau_2$ are varied independently. 
The diagonal entries correspond to matched auxiliary noise levels, and the highlighted entry corresponds to the default setting $\tau_1=\tau_2=1.25\sigma$. 
The off-diagonal entries show that ACR-ES remains effective even when $\tau_1\neq \tau_2$.

Moreover, we test whether ACR-ES requires the auxiliary corrupted references to have the same noise type as the observed image.
In this study, the observed image $y$ is fixed as the same Gaussian-corrupted input, while the auxiliary references $y_1$ and $y_2$ are generated using Gaussian, Poisson, or impulse noise.
Since the auxiliary references participate in the ACR-ES construction, changing their noise type may induce a different optimization trajectory; therefore, the oracle is computed separately for each row.
As shown in Table~\ref{tab:acr_noise_type_set3}, Poisson auxiliary references remain effective and achieve a gap comparable to the matched Gaussian setting on average.
Impulse auxiliary references are less stable, mainly due to failures on Starfish and Butterfly, but still work well on Leaves.
These results suggest that ACR-ES is reasonably robust to moderate auxiliary noise-type mismatch, although impulse-type auxiliary corruptions can be less reliable.

Table~\ref{tab:acr_fixed_gaussian_aux_set3} studies a reversed noise-type mismatch setting, where the auxiliary references $y_1$ and $y_2$ are fixed to Gaussian-corrupted observations, while the observed image $y$ is corrupted by Gaussian, Poisson, or impulse noise.
The Gaussian case is the matched setting, and the Poisson and impulse cases test whether ACR-ES remains effective when the observation and auxiliary references have different noise types.
ACR-ES remains reasonably robust under this mismatch: the average gap increases from $0.33$ dB in the matched Gaussian case to $0.49$ dB for Poisson and $0.61$ dB for impulse.
This indicates that ACR-ES does not require an exact match between the noise type of $y$ and that of the auxiliary references, although matched Gaussian references yield the most stable stopping behavior.

These results indicate that ACR-ES is robust to moderate auxiliary-noise scaling and mismatch, and does not require precise tuning of the auxiliary corruption levels.

\begin{table}[t]
\centering
\caption{
Auxiliary noise-type mismatch study of ACR-ES on Set3.
The observed image $y$ is fixed as the same Gaussian-corrupted input with noise level $\sigma=0.26$.
Only the auxiliary corrupted references $y_1$ and $y_2$ vary across rows: the matched Gaussian setting uses noise level $1.25\times0.26$, the Poisson setting uses noise level $1.25\times10$, and the impulse setting uses corruption probability $1.25\times0.1$.
Since different auxiliary references induce different ACR-ES trajectories, the oracle iteration and oracle PSNR are computed separately for each row.
PSNR Gap denotes the difference between the row-specific oracle PSNR and the selected PSNR.
}
\label{tab:acr_noise_type_set3}
\small
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Noise type}
& \multirow{2}{*}{Image}
& \multicolumn{3}{c}{ACR-ES}
& \multicolumn{2}{c}{\cellcolor{gray!10}Oracle}
& \multirow{2}{*}{$\Delta$ Gap} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-7}
&
& Iter.
& PSNR $\uparrow$
& Gap $\downarrow$
& \cellcolor{gray!10}Iter.
& \cellcolor{gray!10}PSNR $\uparrow$
& \\
\midrule

\multirow{4}{*}{Gaussian}
& Starfish
& 1026
& 21.50
& 0.18
& \cellcolor{gray!10}1437
& \cellcolor{gray!10}21.68
& -- \\
& Butterfly
& 872
& 22.00
& 0.25
& \cellcolor{gray!10}1081
& \cellcolor{gray!10}22.25
& -- \\
& Leaves
& 1101
& 20.39
& 0.31
& \cellcolor{gray!10}1580
& \cellcolor{gray!10}20.70
& -- \\
& \textit{Average}
& --
& 21.29($\pm$0.82)
& 0.25($\pm$0.07)
& --
& \cellcolor{gray!10}21.54($\pm$0.78)
& -- \\
\midrule

\multirow{4}{*}{Poisson}
& Starfish
& 2193
& 22.25
& 0.32
& \cellcolor{gray!10}1674
& \cellcolor{gray!10}22.56
& 0.13 \\
& Butterfly
& 1712
& 23.60
& 0.12
& \cellcolor{gray!10}1451
& \cellcolor{gray!10}23.72
& -0.13 \\
& Leaves
& 2300
& 21.63
& 0.22
& \cellcolor{gray!10}1949
& \cellcolor{gray!10}21.85
& -0.09 \\
& \textit{Average}
& --
& 22.49($\pm$1.01)
& 0.22($\pm$0.10)
& --
& \cellcolor{gray!10}22.71($\pm$0.94)
& -0.03 \\
\midrule

\multirow{4}{*}{Impulse}
& Starfish
& 2720
& 20.33
& 1.40
& \cellcolor{gray!10}1328
& \cellcolor{gray!10}21.73
& 1.21 \\
& Butterfly
& 2201
& 21.22
& 1.18
& \cellcolor{gray!10}1170
& \cellcolor{gray!10}22.40
& 0.93 \\
& Leaves
& 1863
& 20.53
& 0.22
& \cellcolor{gray!10}1422
& \cellcolor{gray!10}20.75
& -0.09 \\
& \textit{Average}
& --
& 20.69($\pm$0.47)
& 0.93($\pm$0.63)
& --
& \cellcolor{gray!10}21.63($\pm$0.83)
& 0.69 \\

\bottomrule
\end{tabular}}
\end{table}

\begin{table}[t]
\centering
\caption{
Auxiliary noise-type mismatch study of ACR-ES on Set3 with fixed Gaussian auxiliary references.
The observed image $y$ is corrupted by different noise types: Gaussian noise with level $\sigma=0.26$, Poisson noise with level $10$, and impulse noise with corruption probability $0.1$.
The auxiliary corrupted references $y_1$ and $y_2$ are always generated using Gaussian noise with level $1.25\times0.26$.
Since different observed noise types induce different DIP trajectories, the oracle iteration and oracle PSNR are computed separately for each row.
PSNR Gap denotes the difference between the row-specific oracle PSNR and the selected PSNR.
}
\label{tab:acr_fixed_gaussian_aux_set3}
\small
\setlength{\tabcolsep}{4.8pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccc}
\toprule
\multirow{2}{*}{Noise of $y$}
& \multirow{2}{*}{Image}
& \multicolumn{3}{c}{ACR-ES}
& \multicolumn{2}{c}{\cellcolor{gray!10}Oracle}
& \multirow{2}{*}{$\Delta$ Gap} \\
\cmidrule(lr){3-5}
\cmidrule(lr){6-7}
&
& Iter.
& PSNR $\uparrow$
& Gap $\downarrow$
& \cellcolor{gray!10}Iter.
& \cellcolor{gray!10}PSNR $\uparrow$
& \\
\midrule

\multirow{4}{*}{\makecell{Gaussian\\(matched)}}
& Starfish
& 1034
& 21.38
& 0.16
& \cellcolor{gray!10}1291
& \cellcolor{gray!10}21.54
& -- \\
& Butterfly
& 1013
& 22.05
& 0.09
& \cellcolor{gray!10}1288
& \cellcolor{gray!10}22.15
& -- \\
& Leaves
& 843
& 19.90
& 0.73
& \cellcolor{gray!10}1579
& \cellcolor{gray!10}20.63
& -- \\
& \textit{Average}
& --
& 21.11($\pm$1.10)
& 0.33($\pm$0.35)
& --
& \cellcolor{gray!10}21.44($\pm$0.76)
& -- \\
\midrule

\multirow{4}{*}{\makecell{Poisson\\(mismatched)}}
& Starfish
& 962
& 21.86
& 0.53
& \cellcolor{gray!10}1471
& \cellcolor{gray!10}22.39
& 0.37 \\
& Butterfly
& 894
& 22.53
& 0.55
& \cellcolor{gray!10}1412
& \cellcolor{gray!10}23.08
& 0.45 \\
& Leaves
& 1056
& 19.72
& 0.40
& \cellcolor{gray!10}1856
& \cellcolor{gray!10}20.12
& -0.33 \\
& \textit{Average}
& --
& 21.37($\pm$1.47)
& 0.49($\pm$0.08)
& --
& \cellcolor{gray!10}21.87($\pm$1.55)
& 0.16 \\
\midrule

\multirow{4}{*}{\makecell{Impulse\\(mismatched)}}
& Starfish
& 965
& 22.45
& 0.64
& \cellcolor{gray!10}1649
& \cellcolor{gray!10}23.09
& 0.47 \\
& Butterfly
& 886
& 22.76
& 0.63
& \cellcolor{gray!10}1646
& \cellcolor{gray!10}23.39
& 0.54 \\
& Leaves
& 1073
& 21.44
& 0.56
& \cellcolor{gray!10}1855
& \cellcolor{gray!10}22.00
& -0.17 \\
& \textit{Average}
& --
& 22.22($\pm$0.69)
& 0.61($\pm$0.04)
& --
& \cellcolor{gray!10}22.82($\pm$0.73)
& 0.28 \\

\bottomrule
\end{tabular}}
\end{table}



==> sections/Algorithmic_Details.tex <==
\section{Algorithmic Details}
\label{app:algorithm_details}

This appendix records the pseudocode for the three pseudo-reference early stopping criteria introduced in Section~\ref{sec:algorithms}. The main text gives the defining validation curves; the algorithms below make explicit the inputs, selected stopping time, and returned reconstruction.

\begin{algorithm}[h]
\caption{Channel-Similarity Reference Early Stopping (CSR-ES)}
\label{alg:rgb-similarity}
\begin{algorithmic}[1]
\Require Noisy RGB image $y=(y_R,y_G,y_B)$; DIP trajectory $\{\hat x_t\}_{t=1}^T$
\State Compute pairwise channel distances
\begin{equation}\nonumber
    d_{ij}=\frac1n\|y_i-y_j\|^2,
    \qquad i,j\in\{R,G,B\},\ i\ne j.
\end{equation}
\State Select the closest channel pair
\begin{equation}\nonumber
    (i^\star,j^\star)=\arg\min_{i\ne j}d_{ij}.
\end{equation}
\State Evaluate the cross-channel validation curve
\begin{equation}\nonumber
    V_t^{\rm CSR}=\frac1n\|\hat x_{t,i^\star}-y_{j^\star}\|^2.
\end{equation}
\State Select
\begin{equation}\nonumber
    \hat t_{\rm CSR}=\arg\min_{1\le t\le T}V_t^{\rm CSR}.
\end{equation}
\State \Return $\hat x_{\hat t_{\rm CSR}}$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Mask-Reference Early Stopping (MR-ES)}
\label{alg:mask-reference}
\begin{algorithmic}[1]
\Require Noisy image $y$; retention probability $p$; DIP iterations $T$
\State Sample or choose a mask $M\in\{0,1\}^n$ with high retention rate, e.g., $\mathbb P(M_i=1)=p=0.98$, and set $H=1-M$.
\State Train DIP using the masked loss
\begin{equation}\nonumber
    \min_\theta \|M\odot(f_\theta(z)-y)\|^2.
\end{equation}
\State Along the resulting trajectory $\{\hat x_t\}_{t=1}^T$, evaluate only on held-out pixels:
\begin{equation}\nonumber
    V_t^{\rm MR}
    =
    \frac1{\sum_iH_i}
    \|H\odot(\hat x_t-y)\|^2.
\end{equation}
\State Select
\begin{equation}\nonumber
    \hat t_{\rm MR}=\arg\min_{1\le t\le T}V_t^{\rm MR}.
\end{equation}
\State \Return $\hat x_{\hat t_{\rm MR}}$.
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
\caption{Augmented-Channel Reference Early Stopping (ACR-ES)}
\label{alg:aug-channel}
\begin{algorithmic}[1]
\Require Noisy image $y$ with $C$ channels; auxiliary noise scale $\tau$; burn-in $t_0$; DIP iterations $T$
\State 
% Generate two pseudo-copies
% \begin{equation}\nonumber
%     y^{(1)}=y+\zeta_1,
%     \qquad
%     y^{(2)}=y+\zeta_2,
%     \qquad
%     \zeta_1,\zeta_2\sim\mathcal N(0,\tau^2I).
% \end{equation}
Generate two independent corrupted measurements
\begin{equation}\nonumber
    y^{(1)} = \mathrm{Corrupt}(y;\zeta_1),
    \qquad
    y^{(2)} = \mathrm{Corrupt}(y;\zeta_2),
\end{equation}
where $\zeta_1$ and $\zeta_2$ with noise level $\tau$ are user-specified auxiliary independent perturbations following the same corruption model. 
\State Construct the augmented fitting target
\begin{equation}\nonumber
    Y=\operatorname{concat}(y,y^{(1)}).
\end{equation}
\State Train a DIP network with $2C$ output channels to fit $Y$, producing outputs $\hat X_t=f_{\theta_t}(z)$.
\State Let $\hat X_{t,{\rm aux}}$ denote the auxiliary output channels $C+1:2C$. Evaluate
\begin{equation}\nonumber
B_t^{\rm ACR}
=
\frac{
\sum_\omega \|\omega\|^2
\left|
\mathcal F(\hat X_{t,{\rm aux}}-y^{(2)})(\omega)
\right|^2
}{
\sum_\omega
\left|
\mathcal F(\hat X_{t,{\rm aux}}-y^{(2)})(\omega)
\right|^2
}.
\end{equation}
\State Select
\begin{equation}\nonumber
    \hat t_{\rm ACR}=\arg\max_{t\ge t_0}B_t^{\rm ACR}.
\end{equation}
\State \Return the primary reconstruction $\hat x_{\hat t_{\rm ACR}}=\hat X_{\hat t_{\rm ACR},1:C}$.
\end{algorithmic}
\end{algorithm}

Unlike MSE-based stopping rules that search for a minimum, the spectral-bias ACR-ES Algorithm \ref{alg:aug-channel} uses an $\arg\max$ criterion.
This is because the average-frequency score often follows an increase-then-decrease pattern during DIP training.
In early iterations, the network mainly reconstructs low-frequency structures; as training progresses, meaningful higher-frequency details are recovered and the score increases.
After the near-oracle region, further optimization tends to fit noise or unstable artifacts, reducing the reference-consistent spectral concentration.
Thus, the peak of the spectral-bias score marks the transition from useful detail recovery to overfitting and provides an effective stopping indicator.

==> sections/App_Beyond_DIP_Regularization-Parameter_Selection.tex <==
\section{Beyond DIP: Regularization-Parameter Selection}\label{appen: beyond DIP}
\begin{wrapfigure}{r}{0.43\textwidth}
    \centering
    \vspace{-1em}
    \includegraphics[width=0.41\textwidth]{results/ES-L2.png}
    \caption{
    CSR-ES for selecting the quadratic regularization strength.
    The selected value is close to the oracle value. Test image: F16\_GT.png, corrupted with Gaussian noise at level 25/255.
    }
    \label{fig:rgb-pseudo-validation-lambda}
    \vspace{-0.05em}
\end{wrapfigure}
We show an extension of our proposed algorithm to regularization-parameter selection.
Although this paper focuses on early stopping, the proposed reference-based perspective is not limited to selecting a stopping time. More broadly, it can be used to select other regularization parameters along a family of reconstruction estimators. To illustrate this point, consider the classical Tikhonov-type denoising problem
\begin{equation}\nonumber
    \hat x_\lambda
    =
    \arg\min_x
    \frac12\|x-y\|_2^2
    +
    \frac{\lambda}{2}\|\nabla x\|_2^2 ,
\end{equation}
where the regularization strength \(\lambda\) controls the bias--variance trade-off. In the absence of a clean validation image, one can apply the same pseudo-reference principle by selecting two structurally similar RGB channels, denoising one channel, and using the other noisy channel as a reference. Specifically, for the selected channel pair \((i,j)\), we choose
\begin{equation}\nonumber
    \hat\lambda
    \in
    \arg\min_{\lambda}
    \left\|
        \hat x_{\lambda,i} - y_j
    \right\|_2^2 .
\end{equation}
This criterion does not provide an unbiased estimate of the clean reconstruction error, since the two color channels may differ in both signal content and noise realization. Nevertheless, when the selected channels share similar underlying structure and have partially decorrelated noise, the pseudo-validation curve can still track the location of the oracle regularization parameter. This suggests that the proposed framework is better viewed as a general validation-free model-selection principle for reconstruction problems, rather than as a method tied only to DIP early stopping. The specific construction of the pseudo-reference may depend on the inverse problem, the data modality, and the reconstruction algorithm, but the central idea remains the same: use information not directly fitted by the estimator to select the point on a reconstruction or regularization path.





==> sections/App_Theory_for_Channel-Similarity_Reference.tex <==
\section{Theory for Channel-Similarity Reference}
\label{app:csr_theory}

This appendix records the algorithm-specific justification for CSR-ES used in Section~\ref{sec:algorithms}.
We assume $N_R, N_G, N_B$ are zero-mean, mutually
independent, and sub-Gaussian with variance proxy $\sigma^2$. Let
$\hat x_{t,c}$ denote the $c$-channel of the DIP reconstruction at
iteration $t$. The cross-channel validation curve is
\begin{equation}\nonumber
  V_t^{\mathrm{RGB}}
  \;:=\;
  \tfrac{1}{n}\,\|\hat x_{t,i^\star} - y_{j^\star}\|^2.
\end{equation}
Writing $y_c=x_c+N_c$, define
\begin{equation}\nonumber
  \Delta := x_{j^\star}-x_{i^\star},
  \qquad
  R_t := \frac{1}{n}\|\hat x_{t,i^\star}-x_{i^\star}\|^2,
  \qquad
  \rho := \sqrt{\|\Delta\|^2/n}.
\end{equation}

\paragraph{An unconditional controlled-bias guarantee.}
Substituting $y_{j^\star} = x_{i^\star} + \Delta + N_{j^\star}$,
$\hat x_{t,i^\star} - y_{j^\star} = r_t - \Delta - N_{j^\star}$ where
$r_t := \hat x_{t,i^\star} - x_{i^\star}$. Squaring and dividing by $n$,
\begin{equation}\nonumber
\label{eq:csr-decomp}
V_t^{\mathrm{RGB}}
\;=\;
R_t + \rho^2 + \tfrac{1}{n}\|N_{j^\star}\|^2
\;-\; \tfrac{2}{n}\langle r_t, \Delta\rangle
\;-\; \tfrac{2}{n}\langle r_t, N_{j^\star}\rangle
\;+\; \tfrac{2}{n}\langle \Delta, N_{j^\star}\rangle.
\end{equation}
The first term is the reconstruction risk we wish to monitor; the next
two are $t$-independent constants (in expectation, for the latter); the
remaining three cross terms determine whether $V_t^{\mathrm{RGB}}$ tracks
$R_t$ up to a constant offset.

\begin{proposition}[Controlled-bias guarantee, uniform in $t$]
\label{prop:csr-cauchy}
With probability at least $1-\delta$ over $N_{j^\star}$, simultaneously
for all $1 \le t \le T$,
\begin{equation}\nonumber
\begin{aligned}
  \left|\,
    V_t^{\mathrm{RGB}} - \bigl(R_t + \rho^2 + \sigma^2\bigr)
  \,\right|
  \;&\le\;
  2\rho\sqrt{R_t}
  \;+\;
  \left|\tfrac{2}{n}\langle r_t, N_{j^\star}\rangle\right|
  \;\\&+\;
  C\!\left[
    \rho\sigma\sqrt{\frac{\log(T/\delta)}{n}}
    \;+\;
    \sigma^2\!\left(
      \sqrt{\frac{\log(T/\delta)}{n}}
      +
      \frac{\log(T/\delta)}{n}
    \right)
  \right].
  \end{aligned}
\end{equation}
The first term comes from Cauchy--Schwarz on
$\langle r_t, \Delta\rangle$; the second is the residual cross-correlation
between the reconstruction error and the validation noise; the bracketed
terms come from sub-Gaussian concentration of
$\langle \Delta, N_{j^\star}\rangle$ and Hanson--Wright concentration of
$\|N_{j^\star}\|^2 - n\sigma^2$, with a union bound over
$t \in \{1,\dots,T\}$.
\end{proposition}

When $\rho$ is small and the residual cross-correlation
$\tfrac{1}{n}\langle r_t, N_{j^\star}\rangle$ remains small uniformly in
$t$, the validation curve $V_t^{\mathrm{RGB}}$ tracks $R_t$ up to a
$t$-independent additive offset $\rho^2 + \sigma^2$, with concentration
error vanishing in $n$. This justifies the channel-similarity selection
step in Algorithm~\ref{alg:rgb-similarity}: minimizing $\rho$ shrinks
both the constant offset and the trajectory-dependent distortion
$2\rho\sqrt{R_t}$.


\paragraph{Data-dependent channel-pair selection.}
The pair $(i^\star, j^\star)$ in Algorithm~\ref{alg:rgb-similarity} is
selected by minimizing $\tfrac{1}{n}\|y_i - y_j\|^2$ over pairs, which
expands as
\begin{equation}\nonumber
  \tfrac{1}{n}\|y_i - y_j\|^2
  \;=\;
  \tfrac{1}{n}\|x_i - x_j\|^2
  \;+\;
  \tfrac{1}{n}\|N_i - N_j\|^2
  \;+\;
  \tfrac{2}{n}\langle x_i - x_j, N_i - N_j\rangle.
\end{equation}
The selection therefore depends on the noise realizations through the
second and third terms, with typical bias of order $\sigma^2/\sqrt{n}$
arising from conditioning on the rank statistic among three pairs. In
what follows we condition on the selected pair $(i^\star, j^\star)$ and
treat $\Delta$ as deterministic; this is equivalent to ignoring the
$O(\sigma^2/\sqrt{n})$ adaptive-selection bias, which is dominated by
$\rho^2$ and $\sigma^2$ in the regimes of interest. A fully rigorous
treatment would replace expectations over $N_c$ with conditional
expectations given the selection event, at the cost of additional
notation.


\paragraph{An idealized argmin recovery model.}
Under additional assumptions, the residual cross-correlation vanishes in
expectation and the rule recovers the per-channel argmin during the
noise-fitting phase of training.

\begin{assumption}[Reference-channel holdout]
\label{ass:csr-holdout}
The reconstruction $\hat x_{t,i^\star}$ is independent of $N_{j^\star}$.
\end{assumption}

\begin{assumption}[Per-channel overfitting trajectory]
\label{ass:csr-traj}
There exists $t_0$ such that for $t \ge t_0$,
\begin{equation}\nonumber
  \hat x_{t,i^\star} \;\approx\; x_{i^\star} + \alpha_t\, N_{i^\star},
  \qquad \alpha_t \in [0, 1],
\end{equation}
with $\alpha_t$ monotonically increasing in $t$.
\end{assumption}

Assumption~\ref{ass:csr-holdout} does \emph{not} hold for standard
full-RGB DIP, since the network parameters $\theta_t$ are updated using
gradients from all three channels and therefore $\hat x_{t,i^\star}$
depends on $N_{j^\star}$ through shared weights. The assumption holds
exactly if the $j^\star$-channel is excluded from the training loss
(see Remark~\ref{rem:holdout-variant} below), and approximately when
cross-channel gradient leakage is small relative to the risk variation
that separates the desired stopping region from later overfitted iterates.
Empirically, the effectiveness of CSR-ES suggests this term is not
dominant in the tested regimes; we do not attempt to prove such a bound
here. Assumption~\ref{ass:csr-traj} is the per-channel analogue of the
trajectory model used in the shared-noise analysis.

\begin{theorem}[Idealized risk tracking in the noise-fitting phase]
\label{thm:csr-tracking}
Under Assumptions~\ref{ass:csr-holdout} and~\ref{ass:csr-traj}, for
$t \ge t_0$,
\begin{equation}\nonumber
  \mathbb{E}\!\left[V_t^{\mathrm{RGB}}\right]
  \;=\;
  \alpha_t^2 \sigma^2 + \sigma^2 + \rho^2,
  \qquad
  \mathbb{E}[R_t]
  \;=\;
  \alpha_t^2 \sigma^2.
\end{equation}
Both quantities are strictly monotone increasing in $\alpha_t$, and so
on $\{t \ge t_0\}$ they are minimized at the same iterate.
\end{theorem}

\begin{proof}
Under Assumption~\ref{ass:csr-holdout},
$\mathbb{E}\langle r_t, N_{j^\star}\rangle = 0$ since $N_{j^\star}$ is
mean zero and independent of the first factor. Under
Assumption~\ref{ass:csr-traj},
$\mathbb{E}\langle r_t, \Delta\rangle =
\alpha_t \mathbb{E}\langle N_{i^\star}, \Delta\rangle = 0$ since
$\Delta$ depends only on clean channels and $N_{i^\star}$ is mean zero.
Furthermore $\mathbb{E}\langle \Delta, N_{j^\star}\rangle = 0$ and
$\mathbb{E}\|N_{j^\star}\|^2 = n\sigma^2$. Taking expectation in
\eqref{eq:csr-decomp} gives
$\mathbb{E}[V_t^{\mathrm{RGB}}] = \mathbb{E}[R_t] + \rho^2 + \sigma^2$,
with $\mathbb{E}[R_t] = \alpha_t^2 \sigma^2$ from
Assumption~\ref{ass:csr-traj}.
\end{proof}


\paragraph{Scope of Theorem~\ref{thm:csr-tracking}.}
Two limitations deserve emphasis. First, both
$\mathbb{E}[V_t^{\mathrm{RGB}}]$ and $\mathbb{E}[R_t]$ are monotone
increasing on $\{t \ge t_0\}$, so the theorem describes the
noise-fitting phase only. The early-stopping mechanism arises from
combining this with the descending phase of $R_t$ during image fitting,
where the trajectory model does not apply: $V_t^{\mathrm{RGB}}$ is
non-monotone across the full trajectory, decreasing during image
fitting and increasing during noise fitting, with the rule selecting
the transition. Theorem~\ref{thm:csr-tracking} establishes that the
rule does not drift past the transition, but does not by itself
identify the transition.

Second, the theorem requires the idealized holdout
(Assumption~\ref{ass:csr-holdout}) which is not satisfied by standard
full-RGB DIP. The implemented method therefore corresponds to an
approximate version of the theorem in which the residual
cross-correlation
$\tfrac{1}{n}\langle r_t, N_{j^\star}\rangle$ is treated as small
but nonzero. The unconditional Proposition~\ref{prop:csr-cauchy}
applies in either case and provides the nonparametric guarantee that
channel-similarity selection serves to tighten.

\begin{remark}[A holdout variant of the algorithm]
\label{rem:holdout-variant}
The idealized model becomes exact for an explicit holdout variant in
which the $j^\star$-channel is removed from the training loss:
\begin{equation}\nonumber
  \theta_t
  \;\leftarrow\;
  \theta_{t-1} - \eta\,\nabla_\theta
  \sum_{c \neq j^\star} \tfrac{1}{n}\|\hat x_{t-1,c} - y_c\|^2.
\end{equation}
This variant has the cleanest theoretical justification but trains on
only two of the three channels, which may degrade reconstruction
quality. The implemented full-RGB algorithm is the practical compromise;
empirical comparison is left to future work.
\end{remark}

\begin{remark}[Departures from per-channel noise independence]
\label{rem:csr-indep}
Real RGB noise is approximately but not exactly per-channel independent;
demosaicing and sensor characteristics can induce mild cross-channel
correlation. If
$\mathbb{E}\langle N_{i^\star}, N_{j^\star}\rangle = \rho_{ij} n\sigma^2$,
the cross term in Proposition~\ref{prop:csr-cauchy} acquires an
additional contribution of order $\alpha_t \rho_{ij}\sigma^2$, which
shifts the argmin only when $|\rho_{ij}|$ is sizeable. For typical
natural images and standard sensor models, $|\rho_{ij}|$ is small enough
that the present analysis remains a useful approximation.
\end{remark}




